A Case Study of LLM for Automated Vulnerability Repair: Assessing Impact of Reasoning and Patch Validation Feedback

Recent work in automated program repair (APR) proposes the use of reasoning and patch validation feedback to reduce the semantic gap between the LLMs and the code under analysis. The idea has been shown to perform well for general APR, but its effectiveness in other particular contexts remains underexplored. In this work, we assess the impact of reasoning and patch validation feedback to LLMs in the context of vulnerability repair, an important and challenging task in security. To support the evaluation, we present VRpilot, an LLM-based vulnerability repair technique based on reasoning and patch validation feedback. VRpilot (1) uses a chain-of-thought prompt to reason about a vulnerability prior to generating patch candidates and (2) iteratively refines prompts according to the output of external tools (e.g., compiler, code sanitizers, test suite, etc.) on previously-generated patches. To evaluate performance, we compare VRpilot against the state-of-the-art vulnerability repair techniques for C and Java using public datasets from the literature. Our results show that VRpilot generates, on average, 14% and 7.6% more correct patches than the baseline techniques on C and Java, respectively. We show, through an ablation study, that reasoning and patch validation feedback are critical. We report several lessons from this study and potential directions for advancing LLM-empowered vulnerability repair

==> extra.tex <==
\begin{table}[t!]
\setlength{\tabcolsep}{5pt}
\caption{\codexModel{} versus \gptthree. A dash ("-") indicates that no prompt could produce a safe patch in any of the \numQueries\ queries.}
\label{tab:results-rqone}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{cclrrrrrr}
% \libtiff{} & EF01 & n.h. & \%compile & \%safe\\
\toprule
\multirow{2}{*}{Project} & \multirow{2}{*}{Id} & \multirow{2}{*}{Prompt} & \multicolumn{2}{c}{\codex} & \multicolumn{2}{c}{\gptthree} & \multicolumn{2}{c}{Exact Match} \\
 & & & \# compile & \# safe & \# compile & \# safe & \codex & \gptthree\\
\midrule
\multirow{42}{*}{\libtiff{}} & \multirow{6}{*}{EF01} & n.h. & 4 & 3  & 2 & 0 & \multirow{6}{*}{No} & \multirow{6}{*}{Yes}\\
 &  & s.1 & 4 & 2  & 0 & 0 \\
 &  & s.2 & 8 & 4  & 0 & 0 \\
 &  & c. & 44 & 1  & 24 & 14 \\
 &  & c.a. & 49 & 3  & 44 & 28 \\
 &  & c.n. & 48 & 2  & 40 & 4 \\ 
\cmidrule{2-9}
 & \multirow{6}{*}{EF02\_01} & n.h. & 0 & 0  & 0 & 0 & \multirow{6}{*}{--} & \multirow{6}{*}{No}\\
 &  & s.1 & 0 & 0  & 0 & 0 \\
 &  & s.2 & 0 & 0  & 1 & 0 \\
 &  & c. & 4 &  0 & 49 &  26\\
 &  & c.a. & 40 & 0  & 46 & 35 \\
 &  & c.n. & 37 & 0 & 44 & 18 \\ 
\cmidrule{2-9}
 & \multirow{6}{*}{EF02\_02} & n.h. & 50 & 0  & 50 & 0 & \multirow{6}{*}{--} & \multirow{6}{*}{--}\\
 &  & s.1 & 50 & 0  & 50 & 0 \\
 &  & s.2 & 50 & 0  & 50 & 0 \\
 &  & c. & 50 &  0 & 50 & 0 \\
 &  & c.a. & 50 & 0  & 50 & 0 \\
 &  & c.n. & 50 & 0  & 50 & 0 \\ 
\cmidrule{2-9}
 & \multirow{6}{*}{EF07} & n.h. & 0 & 0  & 0 & 0 & \multirow{6}{*}{No} & \multirow{6}{*}{No}\\
 &  & s.1 & 0 & 0  & 0 & 0 \\
 &  & s.2 & 0 & 0  & 0 & 0 \\
 &  & c. & 26 & 3  & 10 & 0 \\
 &  & c.a. & 1 & 0  & 27 & 0 \\
 &  & c.n. & 0 & 0  & 32 & 1 \\ 
\cmidrule{2-9}
 & \multirow{6}{*}{EF08} & n.h. & 31 & 6  & 48 & 0 & \multirow{6}{*}{No} & \multirow{6}{*}{No}\\
 &  & s.1 & 20 & 0  & 44 & 0 \\
 &  & s.2 & 26 & 0  & 44 & 0 \\
 &  & c. & 6 & 0  & 26 & 0 \\
 &  & c.a. & 8 & 2  & 16 & 0 \\
 &  & c.n. & 10 & 2  & 24 & 2 \\ 
\cmidrule{2-9}
 & \multirow{6}{*}{EF09} & n.h. & 0 & 0  & 0 & 0 & \multirow{6}{*}{No} & \multirow{6}{*}{No}\\
 &  & s.1 & 1 & 1  & 1 & 1 \\
 &  & s.2 & 1 & 1  & 0 & 0 \\
 &  & c. & 46 & 41  & 4 & 2 \\
 &  & c.a. & 45 & 9  & 5 & 5 \\
 &  & c.n. & 46 & 16  & 2 & 1 \\ 
\cmidrule{2-9}
 & \multirow{6}{*}{EF010} & n.h. & 16 & 1  & 0 & 0 & \multirow{6}{*}{No} & \multirow{6}{*}{--}\\
 &  & s.1 & 17 & 14  & 0 & 0 \\
 &  & s.2 & 15 & 11  & 0 & 0 \\
 &  & c. & 5 & 0  & 2 & 0 \\
 &  & c.a. & 3 & 0  & 18 & 0 \\
 &  & c.n. & 6 & 1  & 11 & 0 \\ 
\hline
 \multirow{18}{*}{\libxml{}} & \multirow{6}{*}{EF15} & n.h. & 0 & 0  & 0 & 0 & \multirow{6}{*}{No} & \multirow{6}{*}{No}\\
 &  & s.1 & 0 & 0  & 0 & 0 \\
 &  & s.2 & 0 & 0  & 0 & 0 \\
 &  & c. & 10 & 1  & 9 & 0 \\
 &  & c.a. & 23 & 0  & 17 & 2 \\
 &  & c.n. & 25 & 2  & 19 & 2 \\ 
\cmidrule{2-9} 
 & \multirow{6}{*}{EF17} & n.h. & 0 & 0  & 23 & 22 & \multirow{6}{*}{No} & \multirow{6}{*}{Yes}\\
 &  & s.1 & 0 & 0  & 24 & 15 \\
 &  & s.2 & 0 & 0  & 18 & 12 \\
 &  & c. & 5 & 0  & 46 & 44 \\
 &  & c.a. & 0 & 0  & 40 & 34 \\
 &  & c.n. & 6 & 3  & 49 & 36 \\ 
\cmidrule{2-9}
& \multirow{6}{*}{EF18} & n.h. & 0 & 0  & 10 & 0 & \multirow{6}{*}{--} & \multirow{6}{*}{Yes}\\
 &  & s.1 & 2 & 0  & 10 & 0 \\
 &  & s.2 & 5 & 0  & 11 & 0 \\
 &  & c. & 46 & 0  & 47 & 39 \\
 &  & c.a. & 47 & 0  & 46 & 42 \\
 &  & c.n. & 16 & 0  & 49 & 46 \\ 
\hline
 \multirow{12}{*}{\libjpeg{}} & \multirow{6}{*}{EF20} & n.h. & 40 & 0  & 40 & 0 & \multirow{6}{*}{No} & \multirow{6}{*}{No}\\
 &  & s.1 & 24 & 0  & 37 & 0 \\
 &  & s.2 & 32 & 0  & 13 & 0 \\
 &  & c. & 32 & 1  & 5 & 1 \\
 &  & c.a. & 26 & 0  & 11 & 2 \\
 &  & c.n. & 36 & 0  & 5 & 0 \\ 
\cmidrule{2-9}
& \multirow{6}{*}{EF22} & n.h. & 2 & 0  & 0 & 0 & \multirow{6}{*}{--} & \multirow{6}{*}{No}\\
 &  & s.1 & 2 & 0  & 0 & 0 \\
 &  & s.2 & 0 & 0  & 0 & 0 \\
 &  & c. & 29 & 0  & 1 & 1 \\
 &  & c.a. & 38 & 0  & 1 & 0 \\
 &  & c.n. & 35 & 0  & 47 & 0 \\
\midrule
\multicolumn{3}{c}{$\Sigma$} & - & 130  & - & 509 \\
\bottomrule
\end{tabular}
}
\end{table}





% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[h]
\setlength{\tabcolsep}{5pt}
\caption{GPT-3.5 Versus \tname{}}
\bowen{pick the best prompt in Table~\ref{tab:results-rqone}}
\label{tab:results-rqtwo}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{cccccc}
\toprule
\multirow{2}{*}{Project}       & \multirow{2}{*}{Id} & \multicolumn{2}{c}{\gptthree{}} & \multicolumn{2}{c}{\tname{}} \\ 
                               &                     & \%compile                & \%safe                & \%compile               & \%safe              \\ \hline
\multirow{7}{*}{Libtiff}       & EF01                &                          &                       &                         &                     \\
                               & EF02\_01            &                          &                       &                         &                     \\
                               & EF02\_02            &                          &                       &                         &                     \\
                               & EF07                &                          &                       &                         &                     \\
                               & EF08                &                          &                       &                         &                     \\
                               & EF09                &                          &                       &                         &                     \\
                               & EF10                &                          &                       &                         &                     \\ \hline
\multirow{3}{*}{Libxml2}       & EF15                &                          &                       &                         &                     \\
                               & EF17                &                          &                       &                         &                     \\
                               & EF18                &                          &                       &                         &                     \\ \hline
\multirow{2}{*}{Libjpeg-turbo} & EF20                &                          &                       &                         &                     \\
                               & EF22                &                          &                       &                         &                     \\ \bottomrule
\end{tabular}%
}
\end{table}


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[h]
\caption{Ablation Study}
\label{tab:results-rqtwo}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{cccccccccc}
\toprule
\multirow{2}{*}{Project}       & \multirow{2}{*}{Id} & \multicolumn{2}{c}{\tname\{\}} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}\tname\{\} w/o\\ Compilation Error Msg\end{tabular}} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}\tname\{\} w/o\\ Regression Test Result\end{tabular}} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}\tname\{\} w/o\\ Security Test Result\end{tabular}} \\
                               &                     & \%compile               & \%safe              & \%compile                                                 & \%safe                                                & \%compile                                                 & \%safe                                                 & \%compile                                                & \%safe                                                \\ \hline
\multirow{7}{*}{Libtiff}       & EF01                &                         &                     &                                                           &                                                       &                                                           &                                                        &                                                          &                                                       \\
                               & EF02\_01            &                         &                     &                                                           &                                                       &                                                           &                                                        &                                                          &                                                       \\
                               & EF02\_02            &                         &                     &                                                           &                                                       &                                                           &                                                        &                                                          &                                                       \\
                               & EF07                &                         &                     &                                                           &                                                       &                                                           &                                                        &                                                          &                                                       \\
                               & EF08                &                         &                     &                                                           &                                                       &                                                           &                                                        &                                                          &                                                       \\
                               & EF09                &                         &                     &                                                           &                                                       &                                                           &                                                        &                                                          &                                                       \\
                               & EF10                &                         &                     &                                                           &                                                       &                                                           &                                                        &                                                          &                                                       \\ \hline
\multirow{3}{*}{Libxml2}       & EF15                &                         &                     &                                                           &                                                       &                                                           &                                                        &                                                          &                                                       \\
                               & EF17                &                         &                     &                                                           &                                                       &                                                           &                                                        &                                                          &                                                       \\
                               & EF18                &                         &                     &                                                           &                                                       &                                                           &                                                        &                                                          &                                                       \\ \hline
\multirow{2}{*}{Libjpeg-turbo} & EF20                &                         &                     &                                                           &                                                       &                                                           &                                                        &                                                          &                                                       \\
                               & EF22                &                         &                     &                                                           &                                                       &                                                           &                                                        &                                                          &                                                       \\ \bottomrule
\end{tabular}%
}
\end{table}

==> removeme.tex <==
\subsection{\rqtwo{}} 
\label{res:rqtwo}

% Despite the improvement of \codexvr\ when configured with \chatgpt{} instead of \codex{}, results for RQ1 showed that \codexvr\ still performs poorly overall. Motivated by those results, RQ2 compares our proposed technique, \tname\ (Section \ref{technique}), with an \emph{idealized optimal version} of \codexvr\ that is configured with \chatgpt{} and selects the best prompt for a given example, i.e., the prompt that optimizes the metrics for that example (Section~\ref{sec:metrics}). Note that there is no prompt that always performs the best in every case. For example, such idealized version of \codexvr\ uses the prompt "c.a" for the example "EF01" but uses the prompt "c." for the example "EF17" (Table~\ref{tab:results-rqone}). 

\input{rq2_table}

% Table~\ref{tab:results-rqtwo} shows the results of comparing our technique \tname\ with the baseline. We use a star (*) to emphasize the use of such an idealized version of \codexvr\ and use different shades of green colour under column ``Plausible \%'' to indicate low(er) and high(er) percentage values. The stronger the green shade, the higher the percentage.

% We observe that, while the baseline generates plausible answers in 10 out of 12 cases (observe the two cross marks), \textbf{\tname\ generates plausible answers in all 12 examples in the dataset}, i.e., 20\% improvements. Furthermore, the relative number of plausible answers that \tname\ produces is higher than the baseline by a large margin. Our method generates, on average, \textbf{+42\%} more plausible answers than the baseline (\textbf{69.83\% vs. 27.83\%}). 

% We observe that \textbf{the difference between the percentage of plausible patches generated by \tname{} and \codex{} varies} --ranging from \textbf{+4\%} to \textbf{+100\%} in favour of \tname{}-- in all of the examples with one exception, ``EF20''. For this example, the performance of both approaches is indistinguishable in terms of the percentage of plausible. 

% Moreover, we measure the statistical significance of the improvement gained by our approach. To achieve this, we use a paired t-test after checking the normality of our data using the Shapiro-Wilk normality test. The statistical result shows, with high statistical confidence ($p$-value of \textbf{0.002} $<0.05$), that the distributions of data are distinct. Moreover, we measure the effect size using Cohens' $d$ and obtain a magnitude of \textbf{1.24}, which is considered a large effect size ($>0.8$).

% \vspace{2ex}
% \begin{mdframed}[style=mpdframe,frametitle=Answer summary of RQ2]
% Results show that \tname\ performs better than the established comparison baseline, which is an idealized (i.e., stronger) version of \codexvr~\cite{pearce2022examining}. \tname\ generates plausible patches for all of the examples in the benchmark and it generates plausible patches at a much higher rate compared to the baseline~(+42\% increase).
% \end{mdframed} 

\input{rq3_table}


==> scripts/s <==
#!/bin/bash


# script to compute averages for table 3 (results R1).
# assumption: files bla.txt contains the lines with data and there is no macros in the data such as \emph, \textbf.


grep "Codex" bla.tex > codex.txt
grep "chatgpt" bla.tex > chatgpt.txt


function avg() {
    FILE=$1
    for x in {3..8}
    do
        for y in {1..2}
        do
            sed -e 's/&/,/g' $FILE | awk -F ',' -v colid=$x '{print $colid}'  | awk -F '/' -v colid=$y '{print $colid}' > tmp
            SUM=$(paste -sd+ tmp | bc -l)
            NLINES=$(wc -l < tmp)
            AVG=$(bc -l <<< "scale=1; $SUM/$NLINES")
            echo -n "$AVG"
            if [[ $y == 1 ]];
            then
                echo -n "/"
            fi
        done
        if [[ $x != 8 ]];
        then
            echo -n " & "        
        fi
    done
    echo
}

avg codex.txt
avg chatgpt.txt


==> sections/algo.tex <==
\LinesNumberedHidden
\begin{algorithm}[t!]
\bowen{(1.) I do not see anywhere in text link to this pseudocode,
(2. Major) I cannot see the need of this as we already hv and presented overview fig of our technique, so it is highly redundant.
(3) typically, we need to add line numbers to pseudocode so that we can easily link text to the corresponding code line.}
    \SetKwProg{Init}{Initialize}{}{}
    \SetKwInOut{Input}{input}
    \SetKwInOut{Output}{output}
    \Input { generateInitialPrompt, generateFeedbackPrompt, generateFinalPrompt, chatGPT, generatePatch, buildProject, parseLog, runTestSuite}
    \Output {A plausible repair}
    \Init{}{
    $TEMPERATURE = [0,0.25,0.5,0.75,1]$\\
    $QUERY = 5$\\
    $MODEL\_NAME = GPT-3.5-turbo$\\
    $feedback = None$\\
    $changeCode = None$\\
    }
    \For{$t \in TEMPERATURE$} {
    \For{$q \leftarrow 1$ \KwTo $(QUERY + 1)$}{
    \eIf {$q == 1$}{
         fristPrompt = generateInitialPrompt ()\\
    }
    {
        fristPrompt = generateFeedbackPrompt (changeCode, feedback)\\
    }
    $reasoning = chatGPT( fristPrompt, t, MODEL\_NAME)$\\
    $finalPrompt = generateFinalPrompt (fristPrompt, reasoning)$\\
    $answer =  chatGPT( finalPrompt, t, MODEL\_NAME)$\\
    $patch, changeCode = generatePatch (answer)$\\
    compile, log = buildProject(patch)\\
    \eIf{ not compile} {
       feedback = parseLog (log)\\
    }
    {
        pass, log = runTestSuite ()\\
        \eIf{pass}{
            return patch
        }
        {
           feedback = parseLog (log) 
        }
    }
    }
    }
    \caption{\tname{}} %Vulnerability repair using 
\end{algorithm}

==> sections/background.tex <==
\subsection{Terminology}

\marcelo{include terminology here} \ummay{Do we need this subsection? I don't think we have a lot of jargon that needs to be explained}

% \subsection{A Motivating Example}
% \bowen{Key Points:}

% {\leavevmode\color{blue}
% Find ONE example that both \ef{}~\cite{gao2021beyond} (Table 5) and \codexvr{}~\cite{pearce2022examining} fail to generate the correct patch but our approach is capable to do (by adding proper feedback).

% (1) LLM has a great potential usage for vulnerability repair and it overcomes the limitations of static analysis-based approach (show an example which LLM can produce a correct patch but \ef{} \cite{gao2021beyond}) cannot)

% (2) However, the patches generated by GPT model are usually plausible (use the same example and show the patch generated by Zero shot paper) and it's very dangerous to directly be used without further validation. 

% (3) In-context learning is one of the key advantages of LLMs capability and it can be leveraged to address the above-mentioned limitations of the existing solutions by adding proper feedback in prompts.
% \color{black}}





% \bowen{A list of information may potentially or has been proved useful for vulnerability repair, such as regression test result (with structured error msg), security test result (with structured error msg), vulnerability type, etc.}

==> tmp_rq1_table.tex <==
\begin{table}[t!]
\setlength{\tabcolsep}{2pt}
\caption{\emph{Results of RQ1.} Evaluation of \codexvr{} with different LLM models and prompts. We query each triple of example, model, and prompt \numQueries{} times. The notation $x/y$ indicates $x$ \% plausible patches out of $y$ \% patches that compile. (The higher the values of $x$ and $y$ the better.)
% The last row and the last column aggregate results. The last row ("Average") reports the averages of $x$ and the averages of $y$ in a given column.
The last column shows whether or not one or more prompts used with a given model report a plausible patch.
}
\label{tab:results-rqone}
\centering
\vspace{-2ex}
\resizebox{1\columnwidth}{!}{%
\begin{tabular}{ccccccccc}
\hline
\multirow{2}{*}{EF\#}     & \multirow{2}{*}{Model}               & \multicolumn{6}{c}{Prompt}                                                                                                     & \multirow{2}{*}{Pass?} \\ \cline{3-8}
                          &                                      & n.h                 & s.1              & s.2                 & c.                    & \textbf{c.a}                  & c.n               &                        \\ \hline
\multirow{2}{*}{EF01}     & Codex                                & 6/8                 & 4/8              & 8/16                & 2/82                 & 6/98                 & 4/96              & \cmark  \\
                          & \textbf{\chatgpt{}} & 0/4                 & 0/0              & 0/0                 & 28/48                & \textbf{56/88}       & 8/80              & \cmark  \\ \hline
\multirow{2}{*}{EF02\_01} & Codex                                & 0/0                 & 0/0              & 0/0                 & 0/8                  & 0/80                 & 0/74              & \rxmark \\
                          & \textbf{\chatgpt{}} & 0/0                 & 0/0              & 0/2                 & 52/98                & \textbf{70/92}       & 36/88             & \cmark  \\ \hline
\multirow{2}{*}{EF07}     & \textbf{Codex}                       & 0/0                 & 0/0              & 0/0                 & \textbf{6/52}        & 0/2                  & 0/0               & \cmark  \\
                          & \chatgpt{}          & 0/0                 & 0/0              & 0/0                 & 0/20                 & 0/54                 & 2/64              & \cmark  \\ \hline
\multirow{2}{*}{EF08}     & \textbf{Codex}                       & \textbf{12/62}      & 0/40             & 0/52                & 0/12                 & 4/16                 & 4/20              & \cmark  \\
                          & \chatgpt{}          & 0/96                & 0/88             & 0/88                & 0/52                 & 0/32                 & 4/48              & \cmark  \\ \hline
\multirow{2}{*}{EF09}     & \textbf{Codex}                       & 0/0                 & 2/2              & 2/2                 & \textbf{82/92}       & 18/90                & 32/92             & \cmark  \\
                          & \chatgpt{}          & 0/0                 & 2/2              & 0/0                 & 4/8                  & 10/10                & 2/4               & \cmark  \\ \hline
\multirow{2}{*}{EF15}     & Codex                                & 0/0                 & 0/0              & 0/0                 & 2/20                 & 0/46                 & 4/50              & \cmark  \\
                          & \textbf{\chatgpt{}} & 0/0                 & 0/0              & 0/0                 & 0/18                 & 4/34                 & \textbf{4/38}     & \cmark  \\ \hline
\multirow{2}{*}{EF17}     & Codex                                & 0/0                 & 0/0              & 0/0                 & 0/10                 & 0/0                  & 6/12              & \cmark  \\
                          & \textbf{\chatgpt{}} & 44/46               & 30/48            & 24/36               & \textbf{88/92}       & 68/80                & 72/98             & \cmark  \\ \hline
\multirow{2}{*}{EF18}     & Codex                                & 0/0                 & 0/4              & 0/10                & 0/92                 & 0/94                 & 0/32              & \rxmark \\
                          & \textbf{\chatgpt{}} & 0/20                & 0/20             & 0/22                & 78/94                & 84/92                & \textbf{92/98}    & \cmark  \\ \hline
\multirow{2}{*}{EF20}     & Codex                                & 0/80                & 0/48             & 0/64                & 2/64                 & 0/52                 & 0/72              & \cmark  \\
                          & \textbf{\chatgpt{}} & 0/80                & 0/74             & 0/26                & 2/10                 & \textbf{4/22}        & 0/10              & \cmark  \\ \hline
\multirow{2}{*}{EF22}     & Codex                                & 0/4                 & 0/4              & 0/0                 & 0/58                 & 0/76                 & 0/70              & \rxmark \\
                          & \textbf{\chatgpt{}} & 0/0                 & 0/0              & 0/0                 & \textbf{2/2}         & 0/2                  & 0/94              & \cmark  \\ \hline
%\multirow{2}{*}{Average}  & Codex & 1.6/23.8 & 2.8/20.0 & 2.6/22.8 & 7.8/50.0 & 2.3/55.0 & 4.3/52.5 & 7/10\\
                         % & \chatgpt{} &  3.6/28.8 & 2.6/27.6 & 2.0/22.8 & 21.1/45.5 & \textbf{24.6}/53.5 & 18.3/62.0 & 10/10 \\ \hline
\multirow{2}{*}{Average}  & Codex & 1.8/15.4 & 0.6/10.6 & 1.0/14.4 & 9.4/49.0 & 2.8/55.4 & 5.0/51.8 & 7/10\\
                          & \chatgpt{} &  4.4/24.6 & 3.2/23.2 & 2.4/17.4 & 25.4/44.2 & \textbf{29.6}/50.6 & 22.0/62.2 & 10/10 \\ \hline
\end{tabular}
}
\end{table}


==> utils.tex <==
\usepackage{microtype}

% comment
\usepackage{colortbl}
% \usepackage[table]{xcolor}
\usepackage{booktabs}

\makeatletter
\let\old@mkpream\@mkpream
\def\@mkpream{%
\ifx\CT@drsc@\relax\else\let\CT@drsc@ @\fi
\let\CT@arc@\relax
\old@mkpream}
\let\Bbbk\relax 

%\usepackage[showframe=true]{geometry}
\usepackage{enumitem}

\usepackage{amsmath,amssymb}
\usepackage{fontawesome} % thumbs down
\usepackage{tikz}
\usetikzlibrary{matrix,fit,shapes,calc,positioning,shadows,arrows,shapes,backgrounds,decorations.markings,fadings}
\usepackage[framemethod=tikz]{mdframed}
\mdfdefinestyle{mpdframe}{
    frametitlebackgroundcolor   =black!15,
    frametitlerule              =true,
    roundcorner                 =5pt,
    middlelinewidth             =1pt,
    innermargin                 =0.3cm,
    outermargin                 =0.3cm,
    innerleftmargin             =0.3cm,
    innertopmargin              =0.1cm,
    innerbottommargin           =0.1cm
}

\newcommand{\CodeIn}[1]{\texttt{#1}}

\newcommand{\Fix}[1]{{\sf\small$\blacktriangleright$\textit{\color{red} #1}$\blacktriangleleft$}}

\newcommand{\basicalert}[3]{\fbox{\bfseries\sffamily\scriptsize\color{#3} #1}{\sf\small$\blacktriangleright$\textit{\color{red} #2}$\blacktriangleleft$}}

\definecolor{mygreen}{rgb}{0,0.6,0}
\definecolor{mygray}{rgb}{0.5,0.5,0.5}
\definecolor{mymauve}{rgb}{0.58,0,0.82}

\newcommand{\blue}[1]{\textcolor{blue}{#1}}

\newcommand{\bowen}[1]{\basicalert{Bowen:~}{#1}{blue}}
\newcommand{\marcelo}[1]{\basicalert{Marcelo:~}{#1}{mygreen}}
\newcommand{\ummay}[1]{\basicalert{Ummay:~}{#1}{mymauve}}

\newcommand{\gptthree}{GPT-3.5}
\newcommand{\codex}{Codex}
\newcommand{\codexModel}{codex-cushman-001}
\newcommand{\tname}{\textsc{VRpilot}}
\newcommand{\numQueries}{50}
\newcommand{\numVulExtractFix}{ten}

\newcommand{\matit}[1]{$\mathit{#1}$}

%% names
\newcommand{\vjfix}{\textsc{VjFix}}
\newcommand{\ef}{\textsc{ExtractFix}}
\newcommand{\vjbench}{\textsc{VjBench}}
\newcommand{\vulfourj}{\textsc{Vul4j}}
\newcommand{\newmodel}{\textsc{ChatGPT}}
\newcommand{\chatgpt}{\newmodel{}}
\newcommand{\codexvr}{\textsc{CodexVR}}
\newcommand{\efdata}{\textsc{ExtractFixData}}


\newcommand{\libtiff}{libtiff}
\newcommand{\libxml}{libxml2}
\newcommand{\libjpeg}{libjpeg-turbo}

\newcommand{\rqone}{RQ1: What is the impact of the base LLM and prompt selection on the state-of-the-art technique for VR?}
\newcommand{\rqtwo}{RQ2: How does \tname\ compare against the baseline?}
\newcommand{\rqthree}{RQ3: How do the different components affect the performance of \tname{}?}

%% numbers
\newcommand{\numExamples}{10}


% table
\usepackage{multirow}
\usepackage{graphicx}
% \usepackage{booktabs} % for nice table rules

\newcommand{\gcmark}{{\color{black}\cmark}}
\newcommand{\rxmark}{{\color{red}\xmark}}


% \usepackage{cite}
% \usepackage{amsmath,amsfonts}
% \usepackage{algorithmic}
% \usepackage{graphicx}
% \usepackage{textcomp}
% \def\BibTeX{{\rm B\kern-.05em{\sc i\kern-.025em b}\kern-.08em
%     T\kern-.1667em\lower.7ex\hbox{E}\kern-.125emX}}


\usepackage{pifont}% http://ctan.org/pkg/pifont
\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%

\usepackage[font=footnotesize]{caption, subcaption}
\usepackage[linesnumbered,ruled,vlined]{algorithm2e}


% % \usepackage[svgnames]{xcolor}
% %% hyperlinks
% \usepackage[utf8]{inputenc}
% \usepackage[english]{babel}
% \usepackage{hyperref}
% \hypersetup{
%     colorlinks=true,
%     linkcolor=blue,
%     anchorcolor=blue,
%     filecolor=blue,      
%     citecolor=blue,
%     urlcolor=blue
% }

% \usepackage{lineno}
% \usepackage{subcaption}
% %\usepackage[type1]{libertine}
% \usepackage{lipsum}% http://ctan.org/pkg/lipsum
% \usepackage{algorithm}% http://ctan.org/pkg/algorithm
% \usepackage[noend]{algpseudocode}% http://ctan.org/pkg/algorithmicx


% \usepackage{graphicx}
% \usepackage[compatibility=false]{caption}% http://ctan.org/pkg/caption
% \usepackage{booktabs}
% %% Apparently, there is a conflict with this package and acmart. -Marcelo
% \usepackage{cite}
\usepackage{url}
% \usepackage{multirow}
% \usepackage{pgfplots}
% \usepackage{tikz}
% \usetikzlibrary{matrix,fit,shapes,calc,positioning,shadows,arrows,shapes,backgrounds,decorations.markings,fadings}
% \usepackage[framemethod=tikz]{mdframed}
% \mdfdefinestyle{mpdframe}{
%     frametitlebackgroundcolor   =black!15,
%     frametitlerule              =true,
%     roundcorner                 =5pt,
%     middlelinewidth             =1pt,
%     innermargin                 =0.3cm,
%     outermargin                 =0.3cm,
%     innerleftmargin             =0.3cm,
%     innerrightmargin            =0.3cm,
%     innertopmargin              =0.1cm,
%     innerbottommargin           =0.1cm
% }



% \usepgfplotslibrary{statistics}
% \usepackage{listings}
% %\usepackage[caption=false, font=footnotesize]{subfig}
% \renewcommand{\ttdefault}{pcr}

% \usepackage{flushend}
\usepackage{balance}
% \usepackage{wrapfig}
% \usepackage{enumitem}
% \usepackage{csquotes}
% \usepackage{color, colortbl}
% \definecolor{Gray}{gray}{0.9}
% \definecolor{cadmiumgreen}{rgb}{0.0, 0.42, 0.24}
% % \usepackage{amsmath,amssymb,amsfonts}

% \usepackage{multirow}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}

% \usepackage[skins]{tcolorbox}

% \usepackage{xfp}
% \usepackage{siunitx}





% \DeclareMathVersion{sans}
% \SetSymbolFont{operators}{sans}{OT1}{cmbr}{m}{n}
% \SetSymbolFont{letters}  {sans}{OML}{cmbrm}{m}{it}
% \SetSymbolFont{symbols}  {sans}{OMS}{cmbrs}{m}{n}

% \lstset{ 
%   mathescape=true,
%   backgroundcolor = \color{white},   % choose the background color; you must add \usepackage{color} or \usepackage{xcolor}; should come as last argument
%   basicstyle = \fontfamily{rm},  % the size of the fonts that are used for the code
%   % mathescape=true,
%   % breakatwhitespace=false,         % sets if automatic breaks should only happen at whitespace
%   breaklines=true,                 % sets automatic line breaking
%   captionpos=b,                    % sets the caption-position to bottom
%   commentstyle=\color{mygreen},    % comment style
%   deletekeywords={...},            % if you want to delete keywords from the given language
%   escapeinside={\%*}{*)},          % if you want to add LaTeX within your code
%   extendedchars=true,              % lets you use non-ASCII characters; for 8-bits encodings only, does not work with UTF-8
%   % firstnumber=1000,                % start line enumeration with line 1000
%   frame=none,	                   % adds a frame around the code
%   keepspaces=true,                 % keeps spaces in text, useful for keeping indentation of code (possibly needs columns=flexible)
%   keywordstyle=\color{blue},       % keyword style
%   % language=Octave,                 % the language of the code
%   morekeywords={*,...},            % if you want to add more keywords to the set
%   numbers=none,                    % where to put the line-numbers; possible values are (none, left, right)
%   numbersep=5pt,                   % how far the line-numbers are from the code
%   numberstyle=\stfamily\bfseries, % the style that is used for the line-numbers
%   rulecolor=\color{black},         % if not set, the frame-color may be changed on line-breaks within not-black text (e.g. comments (green here))
%   showspaces=false,                % show spaces everywhere adding particular underscores; it overrides 'showstringspaces'
%   showstringspaces=false,          % underline spaces within strings only
%   showtabs=false,                  % show tabs within strings adding particular underscores
%   stepnumber=1,                    % the step between two line-numbers. If it's 1, each line will be numbered
%   % stringstyle=\color{mymauve},     % string literal style
%   tabsize=2,	                   % sets default tabsize to 2 spaces
%   title=\lstname                 % show the filename of files included with \lstinputlisting; also try caption instead of title
% }
 
% \newcounter{myalgo}
% \newenvironment{myalgo}[1][]{\refstepcounter{myalgo}\par\medskip\noindent%
%    \textbf{Algorithm~\themyalgo. #1} \rmfamily}{\medskip}

% \usepackage[newfloat]{minted}
% \SetupFloatingEnvironment{listing}{name=Code}


\usepackage{tcolorbox}

% acm template related
% \settopmatter{printacmref=false} % Removes citation information below abstract
% \renewcommand\footnotetextcopyrightpermission[1]{} % removes footnote with conference information in first column


==> vjbench_table.tex <==
% \begin{table}[!t]
% \setlength{\tabcolsep}{3pt}
% % \renewcommand{\arraystretch}{1.3}
% \centering
% \caption{Performance of \tname{} on fixing java vulnerabilities. The values under `Plausible' column denotes the number of plausibly fix vulnerability (at least one patch that passes the test cases) and the values under `Correct' denotes the number of correctly fix vulnerability (at least one patch that is semantically equivalent to human patch)}
% \label{tab:results-vjbench}
% \vspace{-3ex}
% \begin{tabular}{ccccc}
% \toprule
% & \multicolumn{2}{c}{\vjfix} & \multicolumn{2}{c}{\tname}  \\ 
% & Plausible & Correct & Plausible & Correct \\
% \midrule
% VjBench (15)  & 4.6  & 4.0 & \textbf{6.0}  & 5.0 \\
% Vul4j (35)  & 10.9  &  6.2 & \textbf{14.0} & 9.0 \\ 
% \midrule
% Total (50) & 15.5 & 10.2 & \textbf{20.0} & 14.0 \\ 
% \hline
% Compilation Rate (\%)  & \multicolumn{2}{c}{79.7}  & \multicolumn{2}{c}{86.0}  \\ 
% \bottomrule
% \end{tabular}
% % \vspace{-4mm}
% \end{table}

% \resizebox{0.99\columnwidth}{!}{%
% \begin{tabular}{ccccccc}
% \hline
% \multicolumn{1}{l}{} & \multicolumn{3}{c}{Codex}                   & \multicolumn{3}{c}{Vr}                     \\
% \multicolumn{1}{l}{} & Compilation \%        & Plausible & Correct & Compilation \%       & Plausible & Correct \\ \hline
% VjBench (15)         & \multirow{2}{*}{79.7} & 4.6       & 4       & \multirow{2}{*}{86}  & 6         & 5       \\
% Vul4J (35)           &                       & 10.9      & 6.2     &                      & 14        & 9       \\ \hline
% Total (50)           & \multicolumn{1}{l}{}  & 15.5      & 10.2    & \multicolumn{1}{l}{} & 20        & 14     
% \end{tabular}
% }
% \end{table}


